Numerical modeling of fluid flow through porous media (Modelowanie numeryczne transportu plynow przez osrodki porowate)

The aim of the thesis is to present and analyze two particular problems of transport in porous media flow. The first of them is related to the process of saturation of porous building materials. Recently, M. K\"untz and P. Laval\'ee, using a computer model of this process, have concluded that the anomalous diffusion assumption is correct. In this thesis I present an alternative explanation of this results without any refer to anomalous diffusion. The second part of the thesis covers the numerical analysis of the tortuosity of the flow -- one of a very interesting physical macroscopic variables characterizing transport in porous media. (in Polish)

==> back.tex <==
% *************** Back matter ***************

% *******************************************************************************************
% W tym miejscu możesz wyłączyć tworzenie spisu symboli, spisu ilustracji, spisu treŚci
% Możesz także wyłączyć tworzenie skorowidza
% *******************************************************************************************

\backmatter

\normalfont
\clearpage
\input{symbols.tex}

\clearpage
\listoffigures

\clearpage
\listoftables

\footnotesize
\printindex

% *************** Koniec back matter ***************


==> symbols.tex <==
% *************** Spis symboli i skrótów ***************

% ******************************************************************************
% W tym miejscu możesz stworzyĆ własną listę symboli i skrótów.
% Wystarczy jedynie oznaczyć miejsce pierwszego wystąpienia symbolu etykietą
% aby na liście symboli otrzymać numer strony, na której on występuje.
% ******************************************************************************

\chapter{Spis symboli i skrótów}

\begin{center}
\small
\begin{longtable}{lp{3.0in}c}
\toprule
\multicolumn{1}{c}{Abbreviation}
                & \multicolumn{1}{c}{Description}
                                & \multicolumn{1}{c}{Definition}\\ \midrule\addlinespace[2pt] \endhead
\bottomrule\endfoot
DMC                             & dynamiczny koder Markowa
                                & \pref{sym:DMC}\\
LZ77                            & odmiana algorytmu Ziva--Lempela
                                & \pref{sym:LZ77}\\
LZ78                            & odmiana algorytmu Ziva--Lempela
                                & \pref{sym:LZ78}\\
\end{longtable}
\end{center}

% *************** Koniec spisu symboli i skrótów ***************

